Generating Class-Level Integration Tests Using Call Site Information

Search-based approaches have been used in the literature to automate the process of creating unit test cases. However, related work has shown that generated unit-tests with high code coverage could be ineffective, i.e., they may not detect all faults or kill all injected mutants. In this paper, we propose CLING, an integration-level test case generation approach that exploits how a pair of classes, the caller and the callee, interact with each other through method calls. In particular, CLING generates integration-level test cases that maximize the Coupled Branches Criterion (CBC). Coupled branches are pairs of branches containing a branch of the caller and a branch of the callee such that an integration test that exercises the former also exercises the latter. CBC is a novel integration-level coverage criterion, measuring the degree to which a test suite exercises the interactions between a caller and its callee classes. We implemented CLING and evaluated the approach on 140 pairs of classes from five different open-source Java projects. Our results show that (1) CLING generates test suites with high CBC coverage, thanks to the definition of the test suite generation as a many-objectives problem where each couple of branches is an independent objective; (2) such generated suites trigger different class interactions and can kill on average 7.7% (with a maximum of 50%) of mutants that are not detected by tests generated at the unit level; (3) CLING can detect integration faults coming from wrong assumptions about the usage of the callee class (32 for our subject systems) that remain undetected when using automatically generated unit-level test suites.

==> Makefile <==
BASE_NAME = main
INPUTS    = $(wildcard *.tex) $(wildcard sections/*.tex) $(wildcard figures/*.pdf) *.bib

LATEX     = latex
PDFLATEX  = pdflatex
BIBTEX    = bibtex
MAKEINDEX = makeindex

pdf: $(BASE_NAME).pdf
ps: $(BASE_NAME).ps

$(BASE_NAME).pdf: $(BASE_NAME).tex $(INPUTS)
	$(PDFLATEX) $<
	$(BIBTEX) $(BASE_NAME)
	$(PDFLATEX) $<
	$(PDFLATEX) $<

$(BASE_NAME).ps: $(BASE_NAME).tex
	$(LATEX) $<
	$(BIBTEX) $(BASE_NAME)
	$(LATEX) $<
	$(LATEX) $<

once:
	$(PDFLATEX) $(BASE_NAME)

clean:
	rm -f $(BASE_NAME)*.ps $(BASE_NAME)*.dvi *.log \
	      *.aux *.blg *.toc *.brf *.ilg *.ind \
	      missfont.log $(BASE_NAME)*.bbl $(BASE_NAME)*.pdf $(BASE_NAME)*.out \
		  $(BASE_NAME)*.lof $(BASE_NAME)*.lot

TAG=submission-major-1-TSE

diffs:
	mkdir -p diffs-tmp/ && \
	git latexdiff $(TAG) HEAD --main $(BASE_NAME).tex --bibtex --tmpdirprefix TSE/diffs-tmp/


==> tables/cbc-table.tex <==
\begin{tabular}{ l c | rrrr | ccccc }
\hline 
\textbf{Project} & \textbf{Pairs} & \multicolumn{4}{c|}{\textbf{Coupled branches}} & \multicolumn{5}{c}{\textbf{Couples branches coverage}} \\ 
  &   & min & $\overline{\text{count}}$ & $\sigma$ & max & min & $\overline{\text{cov}}$ & $\sigma$ & CI & max \\ 
\hline 
closure & 26 & 4 & 10,542 & 16,764 & 60,754 & 0.00 & 0.23 & 0.27 & [0.21,0.25] & 0.82 \\ 
lang & 18 & 2 & 409 & 582 & 1,826 & 0.00 & 0.48 & 0.38 & [0.44,0.52] & 0.98 \\ 
math & 25 & 2 & 294 & 601 & 2,682 & 0.00 & 0.64 & 0.34 & [0.61,0.67] & 0.99 \\ 
mockito & 19 & 2 & 1,248 & 1,957 & 6,929 & 0.00 & 0.35 & 0.34 & [0.32,0.38] & 0.95 \\ 
time & 48 & 2 & 525 & 1,109 & 5,457 & 0.00 & 0.64 & 0.30 & [0.62,0.66] & 0.99 \\ 
\hline 
\textbf{ Total  } & 136 & 2 & 2,483 & 8,376 & 60,754 & 0.00 & 0.50 & 0.36 & [0.49,0.51] & 0.99 \\ 
\end{tabular}

==> tables/mutation-operators-table-randoop.tex <==
\resizebox{0.49\textwidth}{!}{%
\begin{tabular}{ l l | r}
\hline 
  & \textbf{Mutation operator} & \textbf{\# of kills} \\ 
\hline 
1 & \textbf{NonVoidMethodCallMutator} (\textit{RetStaRep}) & 1809 \\ 
2 & NegateConditionalsMutator & 1505 \\ 
3 & RemoveConditionalMutator\_EQUAL\_IF  & 1063 \\ 
4 & InlineConstantMutator & 971 \\ 
5 & RemoveConditionalMutator\_EQUAL\_ELSE & 962 \\ 
6 & \textbf{ReturnValsMutator} (\textit{RetStaRep}) & 944 \\ 
7 & \textbf{ArgumentPropagationMutator} (\textit{FunCalDel}) & 432 \\ 
8 & \textbf{NullReturnValsMutator} (\textit{RetStaRep}) & 428 \\ 
9 & MemberVariableMutator & 379 \\ 
10 & MathMutator & 377 \\ 
11 & \textbf{ConstructorCallMutator} (\textit{FunCalDel}) & 344 \\ 
12 & \textbf{VoidMethodCallMutator} (\textit{FunCalDel}) & 321 \\ 
13 & RemoveConditionalMutator\_ORDER\_IF & 278 \\ 
14 & RemoveConditionalMutator\_ORDER\_ELSE & 248 \\ 
15 & ConditionalsBoundaryMutator & 227 \\ 
16 & \textbf{PrimitiveReturnsMutator} (\textit{RetStaRep}) & 217 \\ 
17 & RemoveSwitchMutator & 198 \\ 
18 & NakedReceiverMutator & 174 \\ 
19 & IncrementsMutator & 119 \\ 
20 & \textbf{EmptyObjectReturnValsMutator} (\textit{RetStaRep}) & 108 \\ 
21 & \textbf{BooleanTrueReturnValsMutator} (\textit{RetStaRep}) & 102 \\ 
22 & RemoveIncrementsMutator & 82 \\ 
23 & \textbf{BooleanFalseReturnValsMutator} (\textit{RetStaRep}) & 49 \\ 
24 & InvertNegsMutator & 31 \\ 
25 & SwitchMutator & 28 \\ 
\end{tabular}
}

==> tables/mutation-operators-table.tex <==
\begin{tabular}{ l l | c}
\hline 
  & \textbf{operator} & \textbf{Number of Occurrences} \\ 
\hline 
1 & org.pitest.mutationtest.engine.gregor.mutators.NonVoidMethodCallMutator & 1984 \\ 
2 & org.pitest.mutationtest.engine.gregor.mutators.NegateConditionalsMutator & 1641 \\ 
3 & org.pitest.mutationtest.engine.gregor.mutators.InlineConstantMutator & 1203 \\ 
4 & org.pitest.mutationtest.engine.gregor.mutators.ReturnValsMutator & 1196 \\ 
5 & org.pitest.mutationtest.engine.gregor.mutators.RemoveConditionalMutator_EQUAL_IF & 1113 \\ 
6 & org.pitest.mutationtest.engine.gregor.mutators.RemoveConditionalMutator_EQUAL_ELSE & 1015 \\ 
7 & org.pitest.mutationtest.engine.gregor.mutators.NullReturnValsMutator & 578 \\ 
8 & org.pitest.mutationtest.engine.gregor.mutators.ArgumentPropagationMutator & 518 \\ 
9 & org.pitest.mutationtest.engine.gregor.mutators.MathMutator & 513 \\ 
10 & org.pitest.mutationtest.engine.gregor.mutators.experimental.MemberVariableMutator & 458 \\ 
11 & org.pitest.mutationtest.engine.gregor.mutators.ConstructorCallMutator & 379 \\ 
12 & org.pitest.mutationtest.engine.gregor.mutators.RemoveConditionalMutator_ORDER_IF & 375 \\ 
13 & org.pitest.mutationtest.engine.gregor.mutators.VoidMethodCallMutator & 374 \\ 
14 & org.pitest.mutationtest.engine.gregor.mutators.RemoveConditionalMutator_ORDER_ELSE & 348 \\ 
15 & org.pitest.mutationtest.engine.gregor.mutators.ConditionalsBoundaryMutator & 323 \\ 
16 & org.pitest.mutationtest.engine.gregor.mutators.PrimitiveReturnsMutator & 309 \\ 
17 & org.pitest.mutationtest.engine.gregor.mutators.experimental.NakedReceiverMutator & 265 \\ 
18 & org.pitest.mutationtest.engine.gregor.mutators.IncrementsMutator & 145 \\ 
19 & org.pitest.mutationtest.engine.gregor.mutators.BooleanTrueReturnValsMutator & 143 \\ 
20 & org.pitest.mutationtest.engine.gregor.mutators.experimental.RemoveIncrementsMutator & 106 \\ 
21 & org.pitest.mutationtest.engine.gregor.mutators.EmptyObjectReturnValsMutator & 71 \\ 
22 & org.pitest.mutationtest.engine.gregor.mutators.BooleanFalseReturnValsMutator & 63 \\ 
23 & org.pitest.mutationtest.engine.gregor.mutators.InvertNegsMutator & 38 \\ 
24 & org.pitest.mutationtest.engine.gregor.mutators.experimental.SwitchMutator & 16 \\ 
25 & RemoveSwitchMutator & 91 \\ 
\end{tabular}

==> tables/mutation-operators.tex <==
\resizebox{0.49\textwidth}{!}{%
\begin{tabular}{ l l | r}
    \hline 
      & \textbf{Mutation operator} & \textbf{\# of kills} \\ 
    \hline 
    1 & \textbf{NonVoidMethodCallMutator} (\textit{RetStaRep}) & 1983 \\ 
    2 & NegateConditionalsMutator & 1638 \\ 
    3 & InlineConstantMutator & 1201 \\ 
    4 & \textbf{ReturnValsMutator} (\textit{RetStaRep}) & 1195 \\ 
    5 & RemoveConditionalMutator\_EQUAL\_IF & 1110 \\ 
    6 & RemoveConditionalMutator\_EQUAL\_ELSE & 1015 \\ 
    7 & \textbf{NullReturnValsMutator} (\textit{RetStaRep}) & 578 \\ 
    8 & \textbf{ArgumentPropagationMutator} (\textit{FunCalDel}) & 518 \\ 
    9 & MathMutator & 513 \\ 
    10 & MemberVariableMutator & 458 \\ 
    11 & \textbf{ConstructorCallMutator} (\textit{FunCalDel}) & 379 \\ 
    12 & RemoveConditionalMutator\_ORDER\_IF & 375 \\ 
    13 & \textbf{VoidMethodCallMutator} (\textit{FunCalDel}) & 374 \\ 
    14 & RemoveConditionalMutator\_ORDER\_ELSE & 348 \\ 
    15 & ConditionalsBoundaryMutator & 322 \\ 
    16 & \textbf{PrimitiveReturnsMutator} (\textit{RetStaRep}) & 309 \\ 
    17 & NakedReceiverMutator & 264 \\ 
    18 & IncrementsMutator & 143 \\ 
    19 & \textbf{BooleanTrueReturnValsMutator} (\textit{RetStaRep}) & 142 \\ 
    20 & RemoveIncrementsMutator & 106 \\ 
    21 & RemoveSwitchMutator & 89 \\
    22 & \textbf{EmptyObjectReturnValsMutator} (\textit{RetStaRep}) & 71 \\ 
    23 & \textbf{BooleanFalseReturnValsMutator} (\textit{RetStaRep}) & 63 \\ 
    24 & InvertNegsMutator & 38 \\ 
    25 & SwitchMutator & 16 \\ 
    \end{tabular}
}
    

==> tables/results-summary-table.tex <==
\begin{tabular}{ l l c | ccccc | ccccc | ccccc }
\hline 
\textbf{Project} & \textbf{Tool} & \textbf{Pairs} & \multicolumn{5}{c}{\textbf{Line coverage}} & \multicolumn{5}{c}{\textbf{Branch coverage}} & \multicolumn{5}{c}{\textbf{Mutation score}} \\ 
  &   &   & min & $\overline{\text{cov}}$ & $\sigma$ & CI & max & min & $\overline{\text{cov}}$ & $\sigma$ & CI & max & min & $\overline{\text{score}}$ & $\sigma$ & CI & max \\ 
\hline 
closure & E.+C. & 26 & 0.00 & 0.45 & 0.31 & [0.42,0.48] & 1.00 & 0.00 & 0.38 & 0.31 & [0.35,0.40] & 1.00 & 0.00 & 0.40 & 0.20 & [0.39,0.42] & 0.81 \\ 
  & E.10 &   & 0.00 & 0.56 & 0.32 & [0.53,0.58] & 1.00 & 0.00 & 0.50 & 0.33 & [0.47,0.53] & 1.00 & 0.00 & 0.41 & 0.18 & [0.40,0.43] & 0.76 \\ 
lang & E.+C. & 18 & 0.00 & 0.86 & 0.24 & [0.84,0.88] & 1.00 & 0.00 & 0.83 & 0.33 & [0.79,0.86] & 1.00 & 0.00 & 0.64 & 0.25 & [0.61,0.66] & 1.00 \\ 
  & E.10 &   & 0.00 & 0.79 & 0.35 & [0.76,0.83] & 1.00 & 0.00 & 0.81 & 0.35 & [0.77,0.84] & 1.00 & 0.00 & 0.60 & 0.30 & [0.57,0.63] & 1.00 \\ 
math & E.+C. & 25 & 0.00 & 0.84 & 0.17 & [0.83,0.86] & 1.00 & 0.00 & 0.81 & 0.25 & [0.79,0.83] & 1.00 & 0.00 & 0.55 & 0.21 & [0.53,0.57] & 0.88 \\ 
  & E.10 &   & 0.00 & 0.88 & 0.21 & [0.86,0.89] & 1.00 & 0.00 & 0.88 & 0.22 & [0.86,0.90] & 1.00 & 0.00 & 0.50 & 0.23 & [0.48,0.51] & 0.87 \\ 
mockito & E.+C. & 20 & 0.00 & 0.64 & 0.31 & [0.61,0.67] & 0.99 & 0.00 & 0.61 & 0.34 & [0.58,0.64] & 1.00 & 0.00 & 0.49 & 0.27 & [0.46,0.52] & 1.00 \\ 
  & E.10 &   & 0.00 & 0.65 & 0.31 & [0.62,0.68] & 1.00 & 0.00 & 0.63 & 0.33 & [0.59,0.66] & 1.00 & 0.00 & 0.42 & 0.25 & [0.40,0.45] & 0.98 \\ 
time & E.+C. & 51 & 0.00 & 0.50 & 0.41 & [0.48,0.53] & 1.00 & 0.00 & 0.44 & 0.40 & [0.42,0.47] & 1.00 & 0.00 & 0.61 & 0.20 & [0.60,0.62] & 1.00 \\ 
  & E.10 &   & 0.00 & 0.51 & 0.42 & [0.48,0.53] & 1.00 & 0.00 & 0.46 & 0.42 & [0.44,0.49] & 0.99 & 0.00 & 0.60 & 0.21 & [0.58,0.61] & 1.00 \\ 
\hline 
\end{tabular}
